Designing the Network Intelligence Stratum for 6G Networks

As network complexity escalates, there is an increasing need for more sophisticated methods to manage and operate these networks, focusing on enhancing efficiency, reliability, and security. A wide range of Artificial Intelligence (AI)/Machine Learning (ML) models are being developed in response. These models are pivotal in automating decision-making, conducting predictive analyses, managing networks proactively, enhancing security, and optimizing network performance. They are foundational in shaping the future of networks, collectively forming what is known as Network Intelligence (NI). Prominent Standard-Defining Organizations (SDOs) are integrating NI into future network architectures, particularly emphasizing the closed-loop approach. However, existing methods for seamlessly integrating NI into network architectures are not yet fully effective. This paper introduces an in-depth architectural design for a Network Intelligence Stratum (NI Stratum). This stratum is supported by a novel end-to-end NI orchestrator that supports closed-loop NI operations across various network domains. The primary goal of this design is to streamline the deployment and coordination of NI throughout the entire network infrastructure, tackling issues related to scalability, conflict resolution, and effective data management. We detail exhaustive workflows for managing the NI lifecycle and demonstrate a reference implementation of the NI Stratum, focusing on its compatibility and integration with current network systems and open-source platforms such as Kubernetes and Kubeflow, as well as on its validation on real-world environments. The paper also outlines major challenges and open issues in deploying and managing NI.

==> bios.tex <==
\begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{paola-soto.jpg}
\end{wrapfigure}\par
\textbf{Author A} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par


% Paola Soto 
% is a Ph.D. researcher at the University of Antwerp - imec. She received her B.Sc. in Electronics and her M.Sc. in Telecommunications Engineering from the University of Antioquia, Colombia, in 2014 and 2018, respectively. Her current research is focused on developing network management strategies using artificial intelligence and machine learning.

% Miguel Camelo, Ph. D
% received a master’s degree in systems and computer engineering (University of Los Andes, Colombia, 2010) and a Ph.D. degree in computer engineering (University of Girona, Spain, 2014). He has authored several papers in international conferences/journals.  He is a Senior Researcher at the University of Antwerp - imec, Belgium, where he leads the research on applied artificial intelligence (AI) in networking. His research interests are in the field of applied AI in communication networks.

% Gines Garcia-Aviles, Ph. D.
% received his Ph.D. degree from the University Carlos III of Madrid. Since January 2021, he has been with i2CAT, where he is currently a research scientist in the AI-driven Systems group. Gines’ research interests are RAN Softwarization, SDN, and NFV technologies for future cellular networks.

% Esteban Municio, Ph. D.
% received his Ph.D. degree from the University of Antwerp at imec (Belgium) in 2020. He then joined imec as a postdoctoral researcher for two years. Since January 2022, he has been with i2CAT, where he is currently a research scientist in the AI-driven Systems group. His research interests are in the field of programmable open networks, Time-Sensitive Networking, and ultra-reliable Industrial IoT.

% Marco Gramaglia, Ph.D. 
% is a professor at UC3M, where he got his Ph.D. in 2012. Dr. Gramaglia's research interests are machine learning applied to 6G Networks, data privacy, and cybersecurity. He has been involved in several projects funded by the European Commission through the 5GPPP and SNS, and he has authored more than 80 peer-reviewed publications.

% Evangelos A. Kosmatos 
% received his Dipl-Ing. degree and his Ph.D. Degree from the School of Electrical and Computer Engineering (ICCS) of the National Technical University of Athens (NTUA), Greece. He has participated in several EU projects. His research interests include 5G, B5G networks, optical networks, IoT networks, middleware, and distributed technologies; he has 20 publications in international journals and 35 publications in international conferences related to these fields

% Nina Slamnik-Kriještorac, Ph.D.
% is a postdoctoral researcher and principal investigator at imec Research Center in Belgium and the University of Antwerp. Her expertise spans network programmability and zero-touch service management in the device-edge-cloud continuum towards 6G. In 2016, she obtained her Master's degree in telecommunications engineering at the Faculty of Electrical Engineering, University of Sarajevo, Bosnia \& Herzegovina. Nina obtained her Ph.D. in 2022, at the University of Antwerp. With a strong background in telecommunications and computer science, Nina has conducted extensive research on advanced network architectures for 5G verticals, focusing on MEC, NFV, and SDN as fundamental technologies. Nina has published numerous research papers in top-tier conferences and journals, and she is currently active in several European projects that are creating 5G enhancements for the transport & logistics sector, with a special focus on designing vertical-tailored services and Edge Network Applications (EdgeApps). Her current research focuses on developing zero-touch techniques for optimizing and automating management and orchestration of EdgeApps within 6G ecosystems, with a particular emphasis on meeting the ultra-low latency and high-reliability requirements of vertical industries such as automotive and transport & logistics.

% Danny De Vleeschauwer, Ph.D.
% received the M.Sc. degree in electrical engineering and the Ph.D. degree in applied sciences from Ghent University, Belgium, in 1985 and 1993, respectively. He currently is a principal research engineer in the Network Automation Department of the Network Systems and Security Research Lab of Nokia Bell Labs in Antwerp, Belgium. Before joining Nokia, he was a Researcher at Ghent University. His early work was on image processing and the application of queuing theory in packet-based networks. His current research interest includes the distributed control of applications over packet-based networks

% Antonio Bazco-Nogueras, Ph.D.
% is currently a post-doctoral researcher at IMDEA Networks Institute, Madrid, Spain. He is the recipient of the Madrid Talent Attraction Grant 2021. He obtained a Ph.D. degree from Sorbonne Université, Paris, France, in collaboration with the Mitsubishi Electric R&D Centre Europe, Rennes, France, in 2019. He was a post-doctoral researcher at EURECOM, Sophia-Antipolis, France, from 2020 to 2021.

% Lidia Fuentes, Ph.D.
% received her MSc degree and a PhD in Computer Science, from the Universidad de Málaga, Spain. She has done all her teaching work at the Department Lenguajes y Ciencias de la Computación since 1993, being the first female Full Professor of this department. She is the head of the CAOSD research group and co-authored over two hundred and fifty publications in Software Engineering and Artificial Intelligence technologies applied to Networking systems and IoT. Examples of these technologies are variability models, machine learning, or self-adaptive systems. She has an important international profile, leading European projects and being a member of program committees of prestigious international conferences.

% Joaquin Ballesteros, Ph.D.
% received the M.Sc. degree in computer science from the University of Malaga, Málaga, Spain, in 2011 and the Ph.D. degree from the University of Malaga (UMA), Málaga, Spain, in 2017. He is currently an Associate Professor with the Department of Computer Science and Programming Languages. His research works include assistive robotics, self-adaptation, and DSPL.

% Andra Lutu, Ph. D.
% is a Senior Researcher at Telefonica Research in Madrid, Spain. Her main research interests lie in the areas of network measurements, interdomain routing and mobile networks, and her work translated into publications in top venues such as ACM MobiCom, ACM SIGCOMM or ACM IMC.

% Luca Cominardi, Ph.D.
% Ph. D. is currently working as Head of Technology at ZettaScale, where he leads R&D activities on Eclipse Zenoh. Previously, he contributed to multiple areas in both academic and industry related to network virtualization and edge computing for 5G systems.

% Ivan Paez, Ph.D.
% Ph. D. is currently working as Project Manager at ZettaScale, where he is involved in EU collaborative R&D projects in areas such as 5G, B5G, Automotive, Robotics, Edge and Fog Computing, and EU-TW 5GPPP initiatives. In the past, he worked as a research engineer in communications protocols for IoT systems, model-based systems engineering, and self-adaptive systems.

% Sergi Alcalá-Marín
% is a Ph.D. student affiliated with the University Carlos III of Madrid (UC3M) and IMDEA Networks Institute. He holds a Master's in Advanced Telecommunications Technologies (MATT) with a specialization in Wireless Networks from the Polytechnic University of Catalonia (UPC) in 2020. His research interests encompass the dynamic fields of Time Series Forecasting, Neural Networks, Network Performance, and 5G technology.

% Livia Elena Chatzieleftheriou, Ph.D.
% is a Juan de la Cierva fellow and post-doctoral researcher at the IMDEA Networks Institute and a part-time Lecturer at the University Carlos III of Madrid (UC3M). She holds an M.Sc. in applied mathematics and a Ph.D. in Computer science. Her current research interests are in online learning and explainable AI for next-generation mobile networks.  

% Andres Garcia-Saavedra, Ph.D.
% received his Ph.D. degree from the University Carlos III of Madrid (UC3M) in 2013. He then joined Trinity College Dublin (TCD), Ireland, as a research fellow until 2015. Currently, he is a Principal Researcher at NEC Laboratories Europe. His research interests lie in applying fundamental mathematics to real-life wireless communication systems.

% Marco Fiore, Ph.D.
% is a Research Professor at IMDEA Networks Institute, Spain, and a co-founder and CTO at Net AI, a UK-based network intelligence company. He received MSc degrees from the University of Illinois at Chicago, USA, and Politecnico of Torino, Italy, a PhD degree from Politecnico di Torino, Italy, and a Habilitation à Diriger des Recherches (HDR) from Université de Lyon, France. Marco has been a Maître de Conférences (Associate Professor) at Institut National des Sciences Appliquées (INSA) de Lyon, France, Associate Researcher at Inria, France, Researcher at Consiglio Nazionale delle Ricerche, Italy, and visiting researcher at Rice University, USA, Universitat Politècnica de Catalunya, Spain, and University College London, UK. He is a former Marie Curie fellow and Royal Society visiting research fellow, a Senior Member of IEEE, and a Member of ACM. Marco's research interests are in subjects at the interface of mobile networks and data science.

